Neural Algorithmic Reasoning for Combinatorial Optimisation

Solving NP-hard/complete combinatorial problems with neural networks is a challenging research area that aims to surpass classical approximate algorithms. The long-term objective is to outperform hand-designed heuristics for NP-hard/complete problems by learning to generate superior solutions solely from training data. Current neural-based methods for solving CO problems often overlook the inherent "algorithmic" nature of the problems. In contrast, heuristics designed for CO problems, e.g. TSP, frequently leverage well-established algorithms, such as those for finding the minimum spanning tree. In this paper, we propose leveraging recent advancements in neural algorithmic reasoning to improve the learning of CO problems. Specifically, we suggest pre-training our neural model on relevant algorithms before training it on CO instances. Our results demonstrate that by using this learning setup, we achieve superior performance compared to non-algorithmically informed deep learning models.

==> diff4e <==
diff --git a/main.tex b/main.tex
index cdf694c..f96f8d4 100644
--- a/main.tex
+++ b/main.tex
@@ -101,7 +101,7 @@ problem has been studied by both theoretical computer scientists
 \cite{balas1983branch, karlin2022slightly} and the ML community 
 \cite{vinyals2015, kool2019attention, joshi2022learning} from different perspectives.
 The former targets the development of hand-engineered approximate
-algorithms, which trade-off optimality for affordable computational
+algorithms, which trade-off optimality for computational
 complexity, whereas the latter's ultimate objective is to learn such
 algorithms instead of manually designing them, i.e. Neural Combinatorial Optimisation (NCO). Hence, learning to solve such a problem and
 pushing the performance beyond that of hand-crafted heuristics, such as the
@@ -115,7 +115,7 @@ many combinatorial problems have natural ``algorithmic'' solutions \cite{christo
 For example, the Christofides' algorithm follows several steps to construct a solution for the TSP. First, it computes the minimum spanning tree (MST) and subsequently applies a matching algorithm to it. In light of this observation, we argue that knowledge of algorithms may be useful also when addressing combinatorial problems through the use of neural networks. Our hypothesis is that a neural network that possesses knowledge of, say, the minimum spanning tree, might be able to generalise better when learning to solve the TSP. In this context, recent advancements in Neural Algorithmic Reasoning (NAR) \cite{velickovic2021neural} neural networks have been shown to be able to effectively learn and reproduce the execution of classical algorithms \cite{velickovic2021neural}, such as the Prim's algorithm \cite{prim1957shortest}. Moreover, current ``neural algorithmic reasoners'' have been proven to be able to learn multiple algorithms at once, exhibiting positive transfer knowledge across them and yielding better quantitative results compared to learning a single algorithm in isolation. 
 
 Motivated by this, in this paper, we explore the applicability of NAR in the
-context of combinatorial optimisation. So far, most of the prior work in neural
+context of NCO. So far, most of the prior work in neural
 algorithmic reasoning focuses on learning algorithms and solving problems
 within the class of complexity of problems solvable in polynomial time, i.e. P.
 In our settings, we aim to solve challenging combinatorial problems, e.g., TSP,
@@ -241,7 +241,7 @@ on $A(\vx)$.
 % \end{equation}
 The encode-process-decode architecture \citep{hamrick2018relational} is
 considered the preferred choice when implementing NAR models
-\cite{velickovic2021neural}. The architecture can be described as a composition
+\cite{velickovic2021neural}. The architecture is a composition
 of three learnable components $net = g \circ p \circ f$, where $f$ and $g$ are
 encoding and decoding functions (usually as simple as linear transformations),
 and $p$ is a suitable neural architecture called {\it processor} that mimics
@@ -439,13 +439,12 @@ which we want to infuse with the knowledge of $\mathcal{B}$. We explored the fol
     \item \textbf{Pre-train and fine-tune (PFT)} -- in the approach above the
         processor weights are frozen. We hypothesise this may not be suitable
         for our P to NP-hard transfer, so we provide results using the same
-        transfer learning technique as above but allowing weights to be changed
-        by gradient descent.
-    \item \textbf{2-processor transfer (2PROC)} -- this technique, proposed by
-        \citet{xhonneux2021transfer} is a combination of the aforementioned
-        two. When transferring from $\gB$ to $\gT$ we use 2 processors -- one is
-        initialised with the pre-trained parameters and kept frozen while the
-        other is randomly initialised and fine-tuned.
+        transfer learning technique as above but allowing weights to be optimised.
+    \item \textbf{2-processor transfer (2PROC)} \cite{xhonneux2021transfer} --
+        this technique is a combination of the aforementioned two. When
+        transferring from $\gB$ to $\gT$ we use 2 processors: one initialised
+        with the pre-trained parameters and kept frozen and another randomly
+        initialised and fine-tuned.
     \item \textbf{Multi-task learning (MTL)} -- this is a setting where the transfer
         from $\gB$ to $\gT$ is performed implicitly by training $\gB$ and $\gT$
         together \emph{but sharing the same processor}. This technique gave the best
@@ -578,7 +577,7 @@ dataset utilized for our models. \textcolor{Red}{For \citet{joshi2022learning}}
 provided, setting the gating to true\footnote{\citet{joshi2022learning} mention
 they use gating on p.5 of their paper}, and defaulting all others. The
 choice of these previous models as benchmarks was motivated by their
-comparable number of parameters to our own model. \textcolor{Red}{For \citet{rampavsek2022recipe} we used the official PyG implementation provided with the same MPNN processor as ours as the \texttt{conv} parameter in order to be able to process edge features}.
+comparable number of parameters to our own model. \textcolor{Red}{For \citet{rampavsek2022recipe} we used the official PyG \citep{Fey/Lenssen/2019} implementation provided with the same MPNN processor as ours as the \texttt{conv} parameter in order to be able to process edge features}.
 
 Furthermore, we included results from deterministic approaches for
 comprehensive evaluation. These deterministic baselines consisted of a greedy
@@ -629,7 +628,7 @@ the tour $\tilde{\pi}$ predicted by the neural network.
 Contrasted to the
 fine-tuned model, which usually tends to achieve the best in-distribution
 validation loss around epoch 13-14, having one frozen processor tends to
-produce only worse and worse examples with training, as evident in \autoref{fig:PFTvsPF}. While for some target
+produce only worse \textcolor{Red}{performance} with training, as evident in \autoref{fig:PFTvsPF}. While for some target
 tasks $\mathcal{T}$ it may be desirable to be as faithful as possible to the base
 $\mathcal{B}$, our experiments suggest this is not the case here.
 % and (b) gives
diff --git a/ref.bib b/ref.bib
index e56000d..7a03394 100644
--- a/ref.bib
+++ b/ref.bib
@@ -614,3 +614,9 @@ eprint = {
   pages={17--60},
   year={1960}
 }
+@inproceedings{Fey/Lenssen/2019,
+  title={Fast Graph Representation Learning with {PyTorch Geometric}},
+  author={Fey, Matthias and Lenssen, Jan E.},
+  booktitle={ICLR Workshop on Representation Learning on Graphs and Manifolds},
+  year={2019},
+}

